OpenSU3D: Open World 3D Scene Understanding using Foundation Models

In this paper, we present a novel, scalable approach for constructing open set, instance-level 3D scene representations, advancing open world understanding of 3D environments. Existing methods require pre-constructed 3D scenes and face scalability issues due to per-point feature vector learning, limiting their efficacy with complex queries. Our method overcomes these limitations by incrementally building instance-level 3D scene representations using 2D foundation models, efficiently aggregating instance-level details such as masks, feature vectors, names, and captions. We introduce fusion schemes for feature vectors to enhance their contextual knowledge and performance on complex queries. Additionally, we explore large language models for robust automatic annotation and spatial reasoning tasks. We evaluate our proposed approach on multiple scenes from ScanNet and Replica datasets demonstrating zero-shot generalization capabilities, exceeding current state-of-the-art methods in open world 3D scene understanding.

==> content/Tables/ablation_studies/sum/clip_models.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\centering
% Table generated by Excel2LaTeX from sheet 'model_comparision (2)'
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{CLIP Models} &   & \multicolumn{5}{c}{Replica \cite{replica}} \\
\cmidrule(lr){3-7}
  &   & mAcc & F-mIoU & AP & AP50 & AP25 \\
\midrule
ViT-L-14 &   & 38.9 & 40.2 & 9.3 & 20.5 & 30.3 \\
ViT-H-14 &   & \textbf{42.6} & \textbf{40.9} & \textbf{9.9} & \textbf{21.6} & \textbf{31.6} \\
%ViT-G-14 &   & \textbf{42.6} & \textbf{46.4} & \textbf{10.4} & 21.1 & 28.4 \\
\bottomrule
\end{tabular}%

\caption{\textbf{Ablation study of CLIP models}. Influence of size of CLIP models  on instance recall performance}

\vspace{-0.5cm}

\label{tab:clip_models}
\end{table}

==> content/Tables/qualitative/sum/gpt_reason.tex <==
\begin{table}[H]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.6}
\centering


% Table generated by Excel2LaTeX from sheet 'label-acc-manual (3)'
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{c}{\multirow{2}[2]{*}{Dataset}} &   & \multicolumn{2}{c}{\multirow{2}[2]{*}{Reasoning \newline{} Acc.}} \\
  &   & \multicolumn{2}{c}{} \\
\midrule
Replica \cite{replica} &   & \multicolumn{2}{c}{0.83} \\[0.1cm]
ScanNet \cite{scannet} &   & \multicolumn{2}{c}{0.68} \\
\bottomrule
\end{tabular}%

\caption{\textbf{Qualitative evaluation of spatial reasoning accuracy}. Overview of spatial reasoning accuracy with GPT4 \cite{gpt4} on the constructed scene, as assessed by human evaluator.}

\label{tab:sum_reason}
\end{table}

==> content/images/method/model.tex <==
\begin{figure}[H]
  \centering
  \modelclip{1}{double sofa}
  
  \modelclip{2}{single sofa}
  

  \caption{\textbf{Heatmaps depicting text-query and scene-feature similarity.} For a given text query (left), comaprision of per instance  cosine similarity results for OW3SU (middle) \& ConceptGraph \cite{conceptgraph} (left) on replica \cite{replica} scenes. Dark red represents maximum similarity, and dark blue lowest. }

  \label{fig:cg_appendix}
\end{figure}

==> content/images/results/queries.tex <==
\begin{figure}[h]
  \centering
  %\begin{tikzpicture}
    % Draw the line
    % \draw[thin, white] (0,0) -- (\linewidth,0);

    % Add the two headings
    %\node at ((0.27*\textwidth, 0.2) {\textbf{Instance Queries}};
    %\node at (3*0.235*\textwidth, 0.2) {\textbf{Affordance Queries}};
    
   % \end{tikzpicture}
  %\twoimagesins{7}{owl}
  \twoimagesins{13}{bottle case}
  %\twoimagesaff{5}{place to sit and work}
  \twoimagesaff{8}{place to cook} \\

    \vspace{0.01cm}

  %\begin{tikzpicture}
    % Draw the line
     %\draw[thin, white] (0,0) -- (\linewidth,0);

    % Add the two headings
    %\node at ((0.27*\textwidth, 0.2) {\textbf{Property Queries}};
    %\node at (3*0.235*\textwidth, 0.2) {\textbf{Relative Queries}};
    
   % \end{tikzpicture}

  
  %\twoimagesprop{3}{black trashcan}
  \twoimagesprop{9}{green towel}
  %\twoimagesrel{1}{place to sit under display}
  \twoimagesrel{12}{green towel next to sink}


\caption{\textbf{Text-Instance Similarity per Query Type.} cosine similarity score of each instance for different  for retrieval with ``Inst.'' (instance), ``Aff.'' (affordance), ``Prop.'' (property), and ``Rel.'' (relative) text queries. \textcolor{yellow!50!white}{\ensuremath{\blacksquare}}: max, \textcolor{blue!30!black}{\ensuremath{\blacksquare}}: min similarity.}


\vspace{-0.3cm}

  \label{fig:method_queries}
\end{figure}
